Preliminary assessment of a cost-effective headphone calibration procedure for soundscape evaluations

The introduction of ISO 12913-2:2018 has provided a framework for standardized data collection and reporting procedures for soundscape practitioners. A strong emphasis was placed on the use of calibrated head and torso simulators (HATS) for binaural audio capture to obtain an accurate subjective impression and acoustic measure of the soundscape under evaluation. To auralise the binaural recordings as recorded or at set levels, the audio stimuli and the headphone setup are usually calibrated with a HATS. However, calibrated HATS are too financially prohibitive for most research teams, inevitably diminishing the availability of the soundscape standard. With the increasing availability of soundscape binaural recording datasets, and the importance of cross-cultural validation of the soundscape ISO standards, e.g.\ via the Soundscape Attributes Translation Project (SATP), it is imperative to assess the suitability of cost-effective headphone calibration methods to maximise availability without severely compromising on accuracy. Hence, this study objectively examines an open-circuit voltage (OCV) calibration method in comparison to a calibrated HATS on various soundcard and headphone combinations. Preliminary experiments found that calibration with the OCV method differed significantly from the reference binaural recordings in sound pressure levels, whereas negligible differences in levels were observed with the HATS calibration.

==> [ICSV'22] Calibration/ICSVstyle.tex <==

% Hastily put together by
% Gergely Takacs
% 13.1.2020
% gergelytakacs@gergelytakacs.com


\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[letterpaper, margin=2cm]{geometry}
\usepackage{color}
\usepackage{graphicx}
\usepackage{subfigure}
\graphicspath{{graphics_fold/}}
\usepackage{epstopdf} %Converts EPS to PDF so PDFLaTeX can be used
\usepackage{times}
\usepackage{etoolbox}
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{fancyhdr}
\usepackage{psfrag}
\usepackage{enumitem}
\usepackage{indentfirst}       % indent the first line of the section and subsection
\usepackage{titlesec}          % customizing the section titles
\usepackage{hyperref}
\usepackage{babel}
\usepackage{listings}
\usepackage{booktabs}
\usepackage{tabularx}


\addto\captionsenglish{\renewcommand{\refname}{REFERENCES}}

% All code, functions, variables are typed like this
\newcommand{\code}[1]{{\lstinline[columns=fixed]{#1}}} %Shorthand for code


%% Added by G. Takacs 27.1.2018 %%

\usepackage[colorinlistoftodos]{todonotes} % Cool To-Do bubbles!
%% Added by G. Takacs 27.1.2018 %%
%\todo{}

\pagestyle{fancy}			        % set default page style
\setlength{\parskip}{0pt}
\setlist{nolistsep}

% custom \thebibliography environment
\makeatletter
\renewcommand*{\@biblabel}[1]{\hfill#1.}
\makeatother

% formatting the head rule and the foot rule
\makeatletter
\patchcmd{\headrule}{\hrule}{\color{blue}\hrule}{}{}
\patchcmd{\footrule}{\hrule}{\color{blue}\hrule}{}{}
\makeatother

% set first page erase the head rule in the first page
\fancypagestyle{firstpage}{
\fancyhead{}
\fancyfoot{}
\fancyfoot[LE,RO]{\small \thepage}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{1.5pt}
}

% custom \maketitle environment
\makeatletter
\def\maketitle{
  \thispagestyle{firstpage}
\vspace*{-11mm}{\centering\includegraphics[width=\textwidth]{header}\\}
  {
   \vspace*{0mm}\fontsize{17}{20}\selectfont\sffamily{}  \noindent \MakeUppercase{\textbf{\@title}}

   \vspace*{3mm}\fontsize{14}{20}\selectfont\rmfamily{} \noindent \@author
  }
}
\makeatother

% setting the standard headers and footers
\fancyhead{}
\fancyfoot{}
\fancyfoot[LE]{\small The 28\textsuperscript{th} International Congress on Sound and Vibration (ICSV28), 24-28 July 2022}
\fancyfoot[RO]{\small The 28\textsuperscript{th} International Congress on Sound and Vibration (ICSV28), 24-28 July 2022\\
\small \thepage}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{1.5pt}

%custom section appearance
\titleformat{\section}
  {\fontsize{14}{14}\normalfont\sffamily\bfseries}
  {\thesection.}{1em}{}                % insert a point after the section number like the original .doc file

\titleformat{\subsection}
  {\normalfont\sffamily\bfseries}
  {\thesubsection}{1em}{}

\titleformat{\subsubsection}
  {\normalfont\sffamily\small}
  {\textit{\thesubsubsection}}{1em}\textit{{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> [ICSV'22] Calibration/tables/SPL.tex <==
\begin{table}[bh!]
\centering
\caption{A-weighted equivalent sound pressure level values of the 27 tracks across in situ, OCV, and HATS calibration methods in dBA. The tracks are listed in the same order as Figure \ref{fig:hats_calib}}
\vspace{\baselineskip}
\setlength{\tabcolsep}{12pt}
\label{tab:SPL}
\begin{tabular}{%
l
*{3}{S[table-format=2.2]}
*{2}{S[table-format=+2.2]}
}
\toprule
{Track ID} & 
$L_\text{A, eq}^{(\text{nom})}$ &
$L_\text{A, eq}^{(\textsc{ocv})}$ &
$L_\text{A, eq}^{(\textsc{hats})}$ &
$\Delta_{\textsc{ocv}}$ &
$\Delta_{\textsc{hats}}$  \\ 
\midrule
E11b  & 85.94 & 88.86 & 85.87 & 2.92  & -0.07 \\
VP01b & 47.95 & 44.70 & 47.86 & -3.25 & -0.10 \\
E02   & 71.69 & 67.40 & 71.51 & -4.29 & -0.17 \\
E01b  & 66.74 & 62.24 & 66.71 & -4.50 & -0.03 \\
OS01c & 76.17 & 71.34 & 76.15 & -4.83 & -0.02 \\
HR01  & 73.42 & 78.54 & 73.40 & 5.12  & -0.01 \\
RPJ01 & 50.57 & 55.98 & 50.98 & 5.41  & 0.41  \\
E05   & 60.55 & 55.06 & 60.40 & -5.49 & -0.15 \\
W09   & 83.06 & 77.07 & 82.96 & -5.99 & -0.09 \\
W16   & 52.45 & 46.39 & 52.82 & -6.06 & 0.37  \\
CT301 & 84.91 & 91.08 & 84.89 & 6.17  & -0.03 \\
E10   & 75.38 & 69.07 & 75.36 & -6.31 & -0.02 \\
E09   & 67.93 & 61.60 & 67.88 & -6.34 & -0.05 \\
W01   & 73.09 & 66.74 & 72.66 & -6.36 & -0.44 \\
OS01d & 83.20 & 76.78 & 83.15 & -6.43 & -0.05 \\
W06   & 61.83 & 55.40 & 61.67 & -6.44 & -0.16 \\
E12b  & 76.24 & 83.03 & 76.15 & 6.79  & -0.09 \\
W15   & 64.92 & 58.06 & 64.84 & -6.86 & -0.08 \\
W22   & 59.82 & 52.72 & 59.51 & -7.10 & -0.31 \\
CG04  & 64.00 & 56.86 & 63.88 & -7.14 & -0.13 \\
N1    & 55.25 & 62.64 & 55.34 & 7.39  & 0.09  \\
W11a  & 66.02 & 58.62 & 65.94 & -7.39 & -0.07 \\
CG07  & 67.04 & 58.97 & 66.96 & -8.07 & -0.08 \\
CG01  & 73.34 & 65.19 & 73.27 & -8.15 & -0.07 \\
W23a  & 59.90 & 51.58 & 59.51 & -8.32 & -0.39 \\
LS06  & 72.30 & 63.59 & 72.27 & -8.71 & -0.03 \\
KT01  & 40.19 & 52.44 & 51.75 & 12.25 & 11.55 \\
\bottomrule
\end{tabular}
\end{table}

==> [ICSV'22] Calibration/tables/hardware.tex <==
\newcolumntype{Z}{>{\raggedright\arraybackslash}p{3.5cm}}
\newcolumntype{H}{>{\raggedright\arraybackslash}p{2cm}}
\newcolumntype{I}{>{\raggedright\arraybackslash}p{2.7cm}}
\newcolumntype{J}{>{\raggedright\arraybackslash}p{4.25cm}}
\newcolumntype{Y}{>{\raggedright\arraybackslash}p{4.25cm}}
\begin{table*}[tb]
\caption{Hardware specifications for calibration, playback, and recording of binaural audio tracks for soundscape evaluations}
\label{tab:hardware}
\setlength{\tabcolsep}{3pt}
\small
\begin{tabularx}{\textwidth}{HZJYI}
\toprule
Type                              
& Recommendations for calibration/playback                             & OCV                                                                  & HATS                                                                 & In situ
\\ \midrule

Headphones 
& Circumaural reference monitor headphones \cite{InternationalTelecommunicationUnionRadiocommunicationSector2015ITU-RSystems}                             
& Beyerdynamic DT 990 Pro & Beyerdynamic DT 990 Pro                     & NA                     
\\ \midrule
Soundcard 
& High-fidelity soundcard                                              
& MOTU Ultralite AVB & MOTU Ultralite AVB                         & NA                     
\\ \midrule
Head and torso simulator        
& Compliant with:
    \begin{itemize}[leftmargin=*]
      \item ITU-T P.58:2013, Section 5.2
      \item ANSI/ASA S3.36:2012, Table 1
      \end{itemize}
& NA
&GRAS 45BB-5 KEMAR Head and Torso
    \begin{itemize}[leftmargin=*]
      \item ANSI: S3.36, S3.25
      \item IEC: 60318-4
      \item ITU-T Rec. P.57 Type~3.3 based on ITU-T Rec. P.58
      \end{itemize}
& HEAD Acoustics BHS II  
\\ \midrule
Analog-to-digital converter (ADC) 
& Any ADC compliant with the head and torso simulator
    \begin{itemize}[leftmargin=*]
      \item Sampling rate: \SI{44.1}{\kilo\hertz} minimum
      \item Resolution: \SI{24}{bits} minimum
      \end{itemize}
& NA
& National Instruments
    \begin{itemize}[leftmargin=*]
          \item NI 9171
          \item NI 9234
          \end{itemize}
& HEAD Acoustics SQobold 
\\ \midrule
Acoustic environment              
& Compliant with ITU-R BS.1116–3, 8.2.1 \cite{InternationalTelecommunicationUnionRadiocommunicationSector2015ITU-RSystems}
& See \cite{Ooi2021AutomationHead} & See \cite{Ooi2021AutomationHead}     
& In situ                
\\
\bottomrule
\end{tabularx}
\end{table*}
